The QCD Phase Transition Region with Domain Wall Quarks

Results will be presented from a study of the QCD transition region using 2+1 flavors of fermions and a dislocation suppressing gauge action on a lattice with temporal extent of 8 and spatial extent 16 (1.9 - 2.7 fm). A series of temperatures from 140 through 200 MeV, separated by 10 MeV have been studied. All the simulations lie on a line of constant physics with 200 MeV pions, realized using domain wall fermion, a chirally symmetric fermion formulation. The chiral condensates, susceptibility, anomalous symmetry breaking and a detailed study of the Dirac spectrum will be described and compared with earlier staggered results.

==> fig/150MeV_norm.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1078,1510){\makebox(0,0)[r]{\strut{} 0.01}}%
      \put(1078,2316){\makebox(0,0)[r]{\strut{} 0.02}}%
      \put(1078,3122){\makebox(0,0)[r]{\strut{} 0.03}}%
      \put(1078,3928){\makebox(0,0)[r]{\strut{} 0.04}}%
      \put(1078,4734){\makebox(0,0)[r]{\strut{} 0.05}}%
      \put(1210,484){\makebox(0,0){\strut{} 0}}%
      \put(1775,484){\makebox(0,0){\strut{} 0.02}}%
      \put(2340,484){\makebox(0,0){\strut{} 0.04}}%
      \put(2905,484){\makebox(0,0){\strut{} 0.06}}%
      \put(3470,484){\makebox(0,0){\strut{} 0.08}}%
      \put(4035,484){\makebox(0,0){\strut{} 0.1}}%
      \put(4600,484){\makebox(0,0){\strut{} 0.12}}%
      \put(5165,484){\makebox(0,0){\strut{} 0.14}}%
      \put(5730,484){\makebox(0,0){\strut{} 0.16}}%
      \put(6295,484){\makebox(0,0){\strut{} 0.18}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}$\rho(\Lambda)$}}}%
      \put(4006,154){\makebox(0,0){\strut{}$\Lambda$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4547){\makebox(0,0)[r]{\strut{}$ m_l+m_{ \mathrm{res} } $}}%
      \csname LTb\endcsname%
      \put(5816,4217){\makebox(0,0)[r]{\strut{}$ m_s+m_{ \mathrm{res} } $}}%
      \csname LTb\endcsname%
      \put(5816,3887){\makebox(0,0)[r]{\strut{}$\Delta<\bar{\psi}\psi>/\pi$}}%
      \csname LTb\endcsname%
      \put(5816,3557){\makebox(0,0)[r]{\strut{}$<\bar{\psi}\psi>/\pi$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./fig/150MeV_norm}}%
    \gplfronttext
  \end{picture}%
\endgroup

